Equivariant Symmetries for Aided Inertial Navigation

Respecting the geometry of the underlying system and exploiting its symmetry have been driving concepts in deriving modern geometric filters for inertial navigation systems (INSs). Despite their success, the explicit treatment of inertial measurement unit (IMU) biases remains challenging, unveiling a gap in the current theory of filter design. In response to this gap, this dissertation builds upon the recent theory of equivariant systems to address and overcome the limitations in existing methodologies. The goal is to identify new symmetries of inertial navigation systems that include a geometric treatment of IMU biases and exploit them to design filtering algorithms that outperform state-of-the-art solutions in terms of accuracy, convergence rate, robustness, and consistency. This dissertation leverages the semi-direct product rule and introduces the tangent group for inertial navigation systems as the first equivariant symmetry that properly accounts for IMU biases. Based on that, we show that it is possible to derive an equivariant filter (EqF) algorithm with autonomous navigation error dynamics. The resulting filter demonstrates superior to state-of-the-art solutions. Through a comprehensive analysis of various symmetries of inertial navigation systems, we formalized the concept that every filter can be derived as an EqF with a specific choice of symmetry. This underlines the fundamental role of symmetry in determining filter performance. This dissertation advances the understanding of equivariant symmetries in the context of inertial navigation systems and serves as a basis for the next generation of equivariant estimators, marking a significant leap toward more reliable navigation solutions.

==> misc/msceqf/matrices.tex <==
\section*{The State Transition Matrix}
\subsection*{The state matrix}
To derive the state matrix ${\mathbf{A}_t}$, and the state transition matrix ${\mathbf{\Phi}}$ we need to choose a set of coordinates and an origin point. Let ${\mathring{\xi}}$ be the an arbitrarily chosen origin point. The state matrix ${\mathbf{A}_t}$ is written
% \begin{equation}
%     \mathbf{A}_t = 
%     \begin{bmatrix}
%         \prescript{}{1}{\mathbf{A}} & \prescript{}{2}{\mathbf{A}} & \Vector{}{0}{9 \times 6} & \Vector{}{0}{9 \times 4}\\
%         \Vector{}{0}{6 \times 9} & \prescript{}{3}{\mathbf{A}} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 4}\\
%         \prescript{}{4}{\mathbf{A}} & \prescript{}{5}{\mathbf{A}} & \prescript{}{6}{\mathbf{A}} & \Vector{}{0}{6 \times 4}\\
%         \Vector{}{0}{4 \times 9} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 4}
%     \end{bmatrix} ,
% \end{equation}
\begin{equation}
    \mathbf{A}_t = 
    \begin{bmatrix}
        \prescript{}{1}{\mathbf{A}} & \prescript{}{2}{\mathbf{A}} & \Vector{}{0}{9 \times 6} & \Vector{}{0}{9 \times 4}\\
        \prescript{}{3}{\mathbf{A}} & \prescript{}{4}{\mathbf{A}} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 4}\\
        \prescript{}{5}{\mathbf{A}} & \prescript{}{6}{\mathbf{A}} & \prescript{}{7}{\mathbf{A}} & \Vector{}{0}{6 \times 4}\\
        \Vector{}{0}{4 \times 9} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 4}
    \end{bmatrix} ,
\end{equation}
where
\begin{align*}
    & \prescript{}{1}{\mathbf{A}} =
    \begin{bmatrix}
        \mathbf{\Psi} - \adMsym{\mathring{\Vector{}{b}{}}} & & \Vector{}{0}{6 \times 3}\\
        \left(\mathring{\Rot{}{}}^T\mathring{\Vector{}{v}{}}\right)^{\wedge} - \hat{b}^{\wedge}\mathring{\Vector{}{b}{\omega}}^{\wedge} & \eye_3 & \Vector{}{0}{3 \times 3}
    \end{bmatrix} ,\\
    & \prescript{}{2}{\mathbf{A}} =
    \begin{bmatrix}
        \eye_3 & \Vector{}{0}{3 \times 3} \\
        \Vector{}{0}{3 \times 3} & \eye_3 \\
        \hat{b}^{\wedge} & \Vector{}{0}{3 \times 3}
    \end{bmatrix} ,\\
    & \prescript{}{3}{\mathbf{A}} = \adMsym{\mathring{\Vector{}{b}{}}}\mathbf{\Psi} - \adMsym{\left(\hat{\delta}^{\vee} + \Vector{}{\theta}{}\right)}\adMsym{\mathring{\Vector{}{b}{}}},\\
    & \prescript{}{4}{\mathbf{A}} = \adMsym{\left(\hat{\delta}^{\vee} + \Vector{}{\theta}{}\right)},\\
    & \prescript{}{5}{\mathbf{A}} = \AdMsym{\mathring{\mathbf{S}}^{-1}}
    \begin{bmatrix}
    -\Vector{}{\psi}{1}^{\wedge} & \Vector{}{0}{3 \times 3} & \Vector{}{0}{3 \times 3}\\
    -\Vector{}{\psi}{3}^{\wedge} - \mathring{\Vector{}{b}{\omega}}^{\wedge}\hat{b}^{\wedge} & \eye_3 & -\Vector{}{\psi}{2}^{\wedge}
    \end{bmatrix},\\
    & \prescript{}{6}{\mathbf{A}} = \AdMsym{\mathring{\mathbf{S}}^{-1}}
    \begin{bmatrix}
        \eye_3 & \Vector{}{0}{3 \times 3}\\
        \hat{b}^{\wedge} & \Vector{}{0}{3 \times 3}
    \end{bmatrix} ,\\
    & \prescript{}{7}{\mathbf{A}} = \adMsym{\left(\AdMsym{\mathring{\mathbf{S}}^{-1}}\Vector{}{\varrho}{}\right)}
\end{align*}
with
\begin{align*}
    & \mathbf{\Psi} =
    \begin{bmatrix}
        \Vector{}{0}{3 \times 3} & \Vector{}{0}{3 \times 3} \\
        g\left(\mathring{\Rot{}{}}^T\ethree\right)^{\wedge} & \Vector{}{0}{3 \times 3}
    \end{bmatrix} ,\\
    % & \Vector{}{\psi}{} = \left(\Vector{}{\psi}{1}, \Vector{}{\psi}{2}\right) = 
    % \begin{bmatrix}
    % \Vector{}{0}{3 \times 1}\\
    % \hat{a}
    % \end{bmatrix} +
    % \begin{bmatrix}
    %     \hat{A} & \Vector{}{0}{3 \times 3}\\
    %     \hat{b}^{\wedge}\hat{A} & \Vector{}{0}{3 \times 3}
    % \end{bmatrix}\Vector{}{w}{} + 
    % \begin{bmatrix}
    %     \eye_{3} & \Vector{}{0}{3 \times 3}\\
    %     \hat{b}^{\wedge} & \Vector{}{0}{3 \times 3}
    % \end{bmatrix}\hat{\delta}^{\vee}
    & \Vector{}{\psi}{1} = \hat{A}\Vector{}{\omega}{} + \delta_{\omega}^{\vee},\\
    & \Vector{}{\psi}{2} = \Vector{}{\psi}{1} - \mathring{\Vector{}{b}{\omega}},\\
    & \Vector{}{\psi}{3} = \hat{a} - \Vector{}{\psi}{1}^{\wedge}\hat{b},\\
    & \Vector{}{\psi}{4} = \hat{a} + \mathring{\Rot{}{}}^T\mathring{\Vector{}{v}{}} - \Vector{}{\psi}{2}^{\wedge}\hat{b} ,\\
    & \Vector{}{\varrho}{} = \left(\Vector{}{\psi}{2}, \Vector{}{\psi}{4}\right)
\end{align*}

\subsection*{The state transition matrix}
The state transition matrix can be approximated as follows
\begin{equation}
    \mathbf{\Phi} = \eye_{25} + \begin{bmatrix}
        \mathbf{\Phi}_{11} & \mathbf{\Phi}_{12} & \Vector{}{0}{9 \times 6} & \Vector{}{0}{9 \times 4}\\
        \mathbf{\Phi}_{21} & \mathbf{\Phi}_{22} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 4}\\
        \mathbf{\Phi}_{31} & \mathbf{\Phi}_{32} & \mathbf{\Phi}_{33} & \Vector{}{0}{6 \times 4}\\
        \Vector{}{0}{4 \times 9} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 4}
    \end{bmatrix}
\end{equation}
with
\begin{align*}
    &\mathbf{\Phi}_{11} = \prescript{}{1}{\mathbf{A}} \Delta T + \left(\prescript{}{1}{\mathbf{A}}^2 + \prescript{}{2}{\mathbf{A}}\prescript{}{3}{\mathbf{A}}\right) \frac{\Delta T^2}{2},\\
    &\mathbf{\Phi}_{12} = \prescript{}{2}{\mathbf{A}} \Delta T + \left(\prescript{}{1}{\mathbf{A}}\prescript{}{2}{\mathbf{A}} + \prescript{}{2}{\mathbf{A}}\prescript{}{4}{\mathbf{A}}\right)\frac{\Delta T^2}{2},\\
    &\mathbf{\Phi}_{21} = \prescript{}{3}{\mathbf{A}} \Delta T + \left(\prescript{}{3}{\mathbf{A}}\prescript{}{1}{\mathbf{A}} + \prescript{}{4}{\mathbf{A}}\prescript{}{3}{\mathbf{A}}\right)\frac{\Delta T^2}{2},\\
    &\mathbf{\Phi}_{22} = \prescript{}{4}{\mathbf{A}} \Delta T + \left(\prescript{}{4}{\mathbf{A}}^2 + \prescript{}{3}{\mathbf{A}}\prescript{}{2}{\mathbf{A}}\right) \frac{\Delta T^2}{2},\\   
    &\mathbf{\Phi}_{31} = \prescript{}{5}{\mathbf{A}} \Delta T + \left(\prescript{}{5}{\mathbf{A}}\prescript{}{1}{\mathbf{A}} + \prescript{}{6}{\mathbf{A}}\prescript{}{3}{\mathbf{A}} + \prescript{}{7}{\mathbf{A}}\prescript{}{5}{\mathbf{A}}\right)\frac{\Delta T^2}{2},\\
    &\mathbf{\Phi}_{32} = \prescript{}{6}{\mathbf{A}} \Delta T + \left(\prescript{}{5}{\mathbf{A}}\prescript{}{2}{\mathbf{A}} + \prescript{}{6}{\mathbf{A}}\prescript{}{4}{\mathbf{A}} + \prescript{}{7}{\mathbf{A}}\prescript{}{6}{\mathbf{A}}\right)\frac{\Delta T^2}{2},\\
    &\mathbf{\Phi}_{33} = \prescript{}{7}{\mathbf{A}} \Delta T + \prescript{}{7}{\mathbf{A}}^2 \frac{\Delta T^2}{2}
\end{align*}

\subsection*{The input matrix}
Assuming ${\bm{\zeta} = \Vector{}{0}{}, \bm{\mu} = \Vector{}{0}{}}$, then the input matrix $\mathbf{B}_t$ is written
\begin{equation}
    \mathbf{B}_t = \begin{bmatrix}
        \prescript{}{1}{\mathbf{B}} & \Vector{}{0}{9 \times 6}\\
        \prescript{}{2}{\mathbf{B}} & - \AdMsym{\hat{B}}\\
        \prescript{}{3}{\mathbf{B}} & \Vector{}{0}{6 \times 6}\\
        \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 6}
    \end{bmatrix}
\end{equation}
where
\begin{align*}
    &\prescript{}{1}{\mathbf{B}} = \AdMsym{\hat{D}}\begin{bmatrix}
        \eye_3 & \Vector{}{0}{3 \times 3}\\
        \Vector{}{0}{3 \times 3} & \eye_3\\
        \Vector{}{0}{3 \times 3} & \Vector{}{0}{3 \times 3}
    \end{bmatrix}\\
    &\prescript{}{2}{\mathbf{B}} = \adMsym{\mathring{\Vector{}{b}{}}}\AdMsym{\hat{B}}\\
    &\prescript{}{3}{\mathbf{B}} = \AdMsym{\mathring{\mathbf{S}}^{-1}\hat{C}}
    \begin{bmatrix}
        \eye_3 & \Vector{}{0}{3 \times 3}\\
        \Vector{}{0}{3 \times 3} & \Vector{}{0}{3 \times 3}
    \end{bmatrix}
\end{align*}

\section*{Initial Covariance}
Let $\mathbf{P}$ be the covariance of the state in the homogeneous space, than the covariance $\mathbf{\Sigma}$ in error coordinates is written
\begin{equation*}
    \mathbf{\Sigma} = \mathbf{D}\mathbf{P}\mathbf{D}^T
\end{equation*}
where
\begin{equation*}
    \mathbf{D} = 
    \begin{bmatrix}
        \AdMsym{\hat{D}} & \Vector{}{0}{9 \times 9} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{4 \times 4}\\
        \begin{matrix}
            \adMsym{\mathring{\Vector{}{b}{}}}\AdMsym{\hat{B}} & \Vector{}{0}{6 \times 3}
        \end{matrix} & \AdMsym{\hat{B}} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{4 \times 4}\\
        \begin{matrix}
                \bm{\Omega} & \Vector{}{0}{6 \times 3} & \bm{\Upsilon}
        \end{matrix} & \Vector{}{0}{6 \times 6} & \AdMsym{\hat{E}} & \Vector{}{0}{4 \times 4}\\
        \Vector{}{0}{6 \times 9} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 6} & \AdMsym{\hat{L}}
    \end{bmatrix}
\end{equation*}
with
\begin{equation*}
    \begin{bmatrix}
            \bm{\Omega} & \bm{\Upsilon}
    \end{bmatrix} = \AdMsym{\mathring{\mathbf{S}}^{-1}\hat{C}}
\end{equation*}

% \section*{Persistent (SLAM) Features}
% \subsection*{Symmetry}

% \subsection*{The state matrix}

% Let ${\mathring{\xi} = \left(\eye, \mathbf{0}, \mathring{\mathbf{S}}, \mathring{\mathbf{K}}, \mathring{\Vector{}{p}{f}}\right)}$ be the chosen origin point. The state matrix ${\mathbf{A}_t}$ is written
% \begin{equation}
%     \mathbf{A}_t = 
%     \begin{bmatrix}
%         \prescript{}{1}{\mathbf{A}} & \prescript{}{2}{\mathbf{A}} & \Vector{}{0}{9 \times 6} & \Vector{}{0}{9 \times 4} & \Vector{}{0}{9 \times 4}\\
%         \Vector{}{0}{6 \times 9} & \prescript{}{3}{\mathbf{A}} & \Vector{}{0}{6 \times 6} & \Vector{}{0}{6 \times 4} & \Vector{}{0}{6 \times 4}\\
%         \prescript{}{4}{\mathbf{A}} & \prescript{}{5}{\mathbf{A}} & \prescript{}{6}{\mathbf{A}} & \Vector{}{0}{6 \times 4} & \Vector{}{0}{9 \times 4}\\
%         \Vector{}{0}{4 \times 9} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 6} & \Vector{}{0}{4 \times 4} & \Vector{}{0}{9 \times 4}\\
%     \end{bmatrix} ,
% \end{equation}

==> misc/msceqf/msceqf.tex <==
\section*{How to Multi State Constraint EqF (MSCEqF)}

\subsection*{MSCEqF state}
Let $\xi_{I} = \left(\Pose{}{}, \Vector{}{b}{}\right) \in \torSE_2(3) \times \R^{6}$ denotes the IMU state of the system, representing the actual state at time $k$.
Let $\xi_{S} = \left(\mathbf{S}, \mathbf{K}\right) \in \torSE(3) \times \torIN(3)$ denotes the camera calibration state of the system.
%Let $\xi_{M} = \Vector{}{p}{f} \in \R^{3}$ denotes the features state of the system.
The full systems state $\xi = \left(\xi_{I}, \xi_{S}\right) \in \mscvio \coloneqq \torSE_2(3) \times \R^{6} \times \torSE(3) \times \torIN(3)$

\emph{Why did not we define cloned IMU poses as part of the state?} It will be clear in the following paragraphs that we can entirely define the cloned states in the symmetry group.

\subsection*{Symmetry}
The symmetry for the IMU state is given by the Semi-Direct symmetry group $\grpSD \coloneqq \left(\SE_2(3) \ltimes \gothse(3)\right)$. The symmetry for the extrinsic calibration state is simply given by $\SE(3)$, while the symmetry for the intrinsic calibration state is given by $\IN$. 

\sloppy
Let's define the $\IN$ group. let ${w, x, y, z \in \MR^{+}}$, then ${L = \left(w, x, y, z\right) \in \IN}$, where ${\IN \coloneqq {\MR^{+}}^{2} \ltimes {\MR^{+}}^{2}}$. The inverse element is written ${L^{-1} = \left(\frac{1}{w}, \frac{1}{x},  -\frac{y}{w}, -\frac{z}{x}\right) \in \IN}$. In its matrix representation:
\begin{equation*}
    L = \begin{bmatrix}
        w & 0 & y\\
        0 & x & z\\
        0 & 0 & 1
    \end{bmatrix}, \qquad 
    L^{-1} = \begin{bmatrix}
        \frac{1}{w} & 0 & - \frac{y}{w}\\
        0 & \frac{1}{x} & -\frac{z}{x}\\
        0 & 0 & 1
    \end{bmatrix} .
\end{equation*}

Therefore, the symmetry group is defined to be $\grpG \coloneqq \left(\SE_2(3) \ltimes \gothse(3)\right) \times \SE(3) \times \IN$.

\sloppy Let ${X = \left(\left(D,\delta\right), E, L\right) \in \grpG}$, with ${D = \left(A, a, b\right) = \left(B, b\right)\in \SE_2(3)}$ such that ${A \in \SO(3),\; a,b \in \R^{3}}$, and ${B = \left(A, a\right) \in \SE(3)}$. Moreover, define $C = \left(A, b\right) \in \SE(3)$, ${E \in \SE(3)}$, and ${L \in \IN}$.
Define ${\phi \AtoB{\grpB \times \mscvio}{\mscvio}}$ as
\begin{equation}\label{eq:phi_se23}
    \phi\left(X, \xi\right) \coloneqq \left(\Pose{}{}D, \AdMsym{B^{-1}}\left(\Vector{}{b}{} - \delta^{\vee}\right), C^{-1}\mathbf{S}E, \mathbf{K}L\right) \in \mscvio .
\end{equation}
Given ${X^{-1} = \left(\left(D^{-1},-\AdMsym{B^{-1}}{\delta}\right), E^{-1}\right) \in \grpG}$, then the inverse action is written
\begin{equation}
    \phi\left(X^{-1}, \xi\right) \coloneqq \left(\Pose{}{}D^{-1}, \AdMsym{B}\Vector{}{b}{} + \delta^{\vee}, C\mathbf{S}E^{-1}, \mathbf{K}L^{-1}\right) \in \mscvio .
\end{equation}

Before discussing the lifted system and deriving the filter matrices, let's consider the symmetry for the case of a single persistent feature. This would be useful to derive normal coordinates for the feature representation that are used in the MSCEqF update as well.

Let ${Q \in \SOT(3)}$, then when persistent feature are included into the state, the symmetry group changes to ${\grpG \coloneqq \left(\SE_2(3) \ltimes \gothse(3)\right) \times \SE(3) \times \IN \times \SOT(3)^k}$, where $k$ is the number of persistent features considered. 
Let ${X = \left(\left(D,\delta\right), E, L, Q\right) \in \grpG}$, then the group action $\phi$ changes according to
\begin{equation}
    \phi\left(X, \xi\right) \coloneqq \left(\Pose{}{}D, \AdMsym{B^{-1}}\left(\Vector{}{b}{} - \delta^{\vee}\right), C^{-1}\mathbf{S}E, \mathbf{K}L, \mathbf{P}\mathbf{S}EQ^{-1}\left(\mathbf{P}\mathbf{S}\right)^{-1}\Vector{}{p}{f}\right) \in \mscvio .
\end{equation}
Given ${X^{-1} = \left(\left(D^{-1},-\AdMsym{B^{-1}}{\delta}\right), E^{-1}, Q^{-1}\right) \in \grpG}$, then the inverse action is written
\begin{equation}
    \phi\left(X^{-1}, \xi\right) \coloneqq \left(\Pose{}{}D^{-1}, \AdMsym{B}\Vector{}{b}{} + \delta^{\vee}, C\mathbf{S}E^{-1}, \mathbf{K}L^{-1}, \mathbf{P}\mathbf{S}E^{-1}Q\left(\mathbf{P}\mathbf{S}\right)^{-1}\Vector{}{p}{f}\right) \in \mscvio .
\end{equation}

\subsection*{Lift and Lifted System}
\begin{align}
    &\Lambda_T = \left(\mathbf{W} - \mathbf{B} + \mathbf{D}\right) + \Pose{}{}^{-1}\left(\mathbf{G} - \mathbf{D}\right)\Pose{}{} ,\\
    &\Lambda_{b} = \adsym{\Vector{}{b}{}^{\wedge}}{\Pi\left(\Lambda_T\right)} - \bm{\tau}^{\wedge} ,\\
    &\Lambda_S = \mathbf{S}^{-1}\Upsilon\left(\Lambda_T\right)\mathbf{S} + \bm{\mu}^{\wedge} ,\\
    &\Lambda_K = \bm{\zeta}^{\wedge} .
\end{align}
%
% In particular, ${\Lambda_{b} = \left(\Lambda_{b_{\omega}}, \Lambda_{b_{a}}\right)}$, with ${\Lambda_{b_{\omega}} = \bw^{\wedge}\left(\ang - \bw\right) - \tauw}$, and ${\Lambda_{b_{a}} = \ba^{\wedge}\left(\ang - \bw\right)  + \bw^{\wedge}\left(\acc - \ba + g\Rot{}{}^{T}\ethree\right) - \taua}$.

\subsection*{How to Impose Multi State Constraint}
Let's for now focus on the unit plane ($Z_1$) projection.
Without the feature as part of the state, and without a symmetry, the measurement is not equivariant, therefore
\begin{equation}
    h\left(\phi_{X}\left(\xi\right)\right) = \mathbf{K}L \pi_{Z_1}\left(E^{-1}\left(\mathbf{P}\mathbf{S}\right)^{-1} * \Vector{}{p}{f}\right)
\end{equation}
Let's consider normal coordinates for the equivariant error ${e = \phi_{\hat{X}}}\left(\xi\right)$, thus ${\varepsilon = \vartheta\left(e\right) = \log_{\grpG}\left(\phi_{\mathring{\xi}}^{-1}\left(e\right)\right)}$.
Define ${\tilde{y} = \varsigma\left(\Vector{}{p}{f}\right) - \varsigma\left(\hatVector{}{p}{f}\right)}$, then, the true feature can be written as ${\Vector{}{p}{f} = \varsigma^{-1}\left(\varsigma\left(\hatVector{}{p}{f}\right) + \tilde{y}\right)}$. 
The measurement model in \equref{visualmeas} can be linearized at ${\varepsilon = \mathbf{0}}$, and ${\tilde{y} = \mathbf{0}}$ as follows:
\begin{equation}
\begin{split}
    h\left(\xi, \Vector{}{p}{f}\right) &= h\left(\phi_{\hat{X}}\left(\vartheta^{-1}\left(\varepsilon\right)\right), \varsigma^{-1}\left(\varsigma\left(\hatVector{}{p}{f}\right) + \tilde{y}\right)\right)\\
    &= h\left(\hat{\xi}, \hatVector{}{p}{f}\right) + \mathbf{C}_t\varepsilon + \mathbf{C}^{f}_t\tilde{y} + \cdots .
\end{split}
\end{equation}
Define ${\Gamma \AtoB{\SE(3)}{\SO(3)}}$ as follows, let ${X \in \SE(3)}$, then ${\Gamma\left(X\right)}$ is written
\begin{equation*}
    \Gamma\left(X\right) \coloneqq \begin{bmatrix}
    \eye_3 & \mathbf{0}_{3 \times 1}
    \end{bmatrix}
    X
    \begin{bmatrix}
    \eye_3\\
    \mathbf{0}_{1 \times 3}
    \end{bmatrix} \quad \forall X \in \SE(3) .
\end{equation*}
Define ${\Xi \AtoB{\R^{3}}{\R{3 \time 4}}}$ as follows, let ${\Vector{}{v}{} \in \R^{3}}$, then ${\Xi\left(\Vector{}{v}{}\right)}$ is written
\begin{equation*}
    \Xi\left(\Vector{}{v}{}\right) \coloneqq \begin{bmatrix}
    v_x & 0 & v_z & 0\\
    0 & v_y & 0 & v_z\\
    0 & 0 & 0 & 0
    \end{bmatrix}
\end{equation*}
Then, let's then compute the ${\mathbf{C}_t}$, and ${\mathbf{C}^{f}_t}$ for different feature parametrization.
\begin{equation}
    \begin{split}
        \mathbf{C}_t\varepsilon &= \Fr{\xi}{\hat{\xi}}h\left(\xi\right)\Fr{e}{\mathring{\xi}}\phi_{\hat{X}}\Fr{\varepsilon}{\mathbf{0}}\vartheta^{-1}\left(\varepsilon\right)\left[\varepsilon\right]\\
        &= \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}\Gamma\left(\hat{E}^{-1}\right)
        \begin{bmatrix}
        \left(\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \hatVector{}{p}{f}\right)^{\wedge} & -\eye_3
        \end{bmatrix}
        \varepsilon_E +
        \mathring{\mathbf{K}}\Xi\left(\hat{L}\pi_{Z_1}\left(\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\hat{E}\right)^{-1} * \hatVector{}{p}{f}\right)\right)
        \varepsilon_K .
        % \\
        % &= \mathring{\mathbf{K}}\hat{L}
        % d_{\pi_{S^{2}}}\Gamma\left(\hat{E}^{-1}\right)
        % \begin{bmatrix}
        % \left({^AE}\hatVector{}{a}{f}\right)^{\wedge} & -\eye_3
        % \end{bmatrix}
        % \varepsilon_E +
        % \mathring{\mathbf{K}}\Xi\left(\hat{L}\pi_{S^2}\left(\hat{E}^{-1}{^AE}\hatVector{}{a}{f}\right)\right)
        % \varepsilon_K\\
        % &= \mathring{\mathbf{K}}\hat{L}
        % d_{\pi_{S^{2}}}\Gamma\left(\hat{E}^{-1}\right)
        % \begin{bmatrix}
        % \left(\hat{E} * \hatVector{}{c}{f}\right)^{\wedge} & -\eye_3
        % \end{bmatrix}
        % \varepsilon_E +
        % \mathring{\mathbf{K}}\Xi\left(\hat{L}\pi_{S^2}\left(\hatVector{}{c}{f}\right)\right)
        % \varepsilon_K .
    \end{split}
\end{equation}

\subsubsection*{Euclidean}
\begin{align}
    &\Vector{}{z}{} = \varsigma\left(\Vector{}{p}{f}\right) = \Vector{}{p}{f} ,\\
    &\Vector{}{p}{f} = \varsigma^{-1}\left(\Vector{}{z}{}\right) = \Vector{}{z}{} .
\end{align}
%
Then the matrix ${\mathbf{C}^{f}_t}$ is written
\begin{equation}
    \begin{split}
        \mathbf{C}^{f}_t\tilde{y} &= 
        \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}
         \Gamma\left(\left(\hat{\mathbf{P}}\hat{\mathbf{S}}\right)^{-1}\right)
        \tilde{y}\\
        &= 
        \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}
         \Gamma\left(\hat{E}^{-1}\right)
        \tilde{y}
    \end{split}
\end{equation}

\subsubsection*{Anchored Inverse Depth}
Let ${^A\mathbf{P} ^A\mathbf{S}}$ be the pose of the anchor, then define the feature in the anchor frame as ${\Vector{}{a}{f} = \left(^A\mathbf{P} ^A\mathbf{S}\right)^{-1} * \Vector{}{p}{f}}$. The anchored inverse depth parametrization is written
\begin{align}
    &\Vector{}{z}{} = \varsigma\left(\Vector{}{p}{f}\right) = \left(\Vector{}{z}{1}, z_2\right) = \left(\left(\frac{a_{f_x}}{a_{f_z}}, \frac{a_{f_y}}{a_{f_z}}\right), \frac{1}{a_{f_z}}\right) ,\\
    &\Vector{}{p}{f} = \varsigma^{-1}\left(\Vector{}{z}{}\right) = \left(^A\mathbf{P} ^A\mathbf{S}\right) * \begin{bmatrix}
        \frac{\Vector{}{z}{1}}{z_2}\\
        \frac{1}{z_2}
    \end{bmatrix} .
\end{align}
%
Then the matrix ${\mathbf{C}^{f}_t}$ is written
\begin{equation}
    \begin{split}
        \mathbf{C}^{f}_t\tilde{y} &= 
        \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}
        \Gamma\left(\left(\hat{\mathbf{P}}\hat{\mathbf{S}}\right)^{-1} {^A\hat{\mathbf{P}}} {^A\hat{\mathbf{S}}}\right)\frac{1}{\hat{z}_2}
        \begin{bmatrix}
            \eye_2 & -\frac{\hatVector{}{z}{1}}{\hat{z}_2}\\
            \Vector{}{0}{1 \times 2} & -\frac{1}{\hat{z}_2}
        \end{bmatrix}
        \tilde{y} \\
        &= 
        \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}
        \Gamma\left({\hat{E}^{-1}} {^A\hat{E}}\right)\frac{1}{\hat{z}_2}
        \begin{bmatrix}
            \eye_2 & -\frac{\hatVector{}{z}{1}}{\hat{z}_2}\\
            \Vector{}{0}{1 \times 2} & -\frac{1}{\hat{z}_2}
        \end{bmatrix}
        \tilde{y}
    \end{split}
\end{equation}

\subsubsection*{Polar parametrization}
Define normal coordinates about ${\mathring{\Vector{}{c}{f}} = \left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}}}$ as follows
\begin{align}
    &\Vector{}{z}{} = \varsigma\left(\Vector{}{p}{f}\right) = \left(\log\left(\frac{\norm{\mathring{\Vector{}{c}{f}}}}{\norm{\Vector{}{c}{f}}}\right), -\arccos\left(\frac{\mathring{\Vector{}{c}{f}}^T\Vector{}{c}{f}}{\norm{\mathring{\Vector{}{c}{f}}}\norm{\Vector{}{c}{f}}}\right)\frac{\mathring{\Vector{}{c}{f}} \times \Vector{}{c}{f}}{\norm{\mathring{\Vector{}{c}{f}} \times \Vector{}{c}{f}}}\right) ,\\
    &\Vector{}{p}{f} = \varsigma^{-1}\left(\Vector{}{z}{}\right) = \left(\mathbf{P}\mathbf{S}\right)\exp_{\SOT(3)}\left(\Vector{}{z}{}^{\wedge}\right)^{-1}\mathring{\Vector{}{c}{f}} ,
\end{align}
where
\begin{align*}
    &\mathring{\Vector{}{c}{f}} = \left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}},\\
    &\Vector{}{c}{f} = \left(\mathbf{P}\mathbf{S}\right)^{-1} * \Vector{}{p}{f}.\\
\end{align*}
%
Then the matrix ${\mathbf{C}^{f}_t}$ is written
\begin{equation}
    \begin{split}
        \mathbf{C}^{f}_t\tilde{y} &= 
        \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}
        \begin{bmatrix}
            \hatVector{}{c}{f}^{\wedge}\mathbf{J}_{L}\left(\arccos\left(\frac{\mathring{\Vector{}{c}{f}}^T\Vector{}{c}{f}}{\norm{\mathring{\Vector{}{c}{f}}}\norm{\Vector{}{c}{f}}}\right)\frac{\mathring{\Vector{}{c}{f}} \times \Vector{}{c}{f}}{\norm{\mathring{\Vector{}{c}{f}} \times \Vector{}{c}{f}}}\right) & -\hatVector{}{c}{f}
        \end{bmatrix}\tilde{y}
        % \\
        % &= \mathring{\mathbf{K}}
        % \hat{L}
        % d_{\pi_{S^{2}}}
        % \begin{bmatrix}
        %     \left(\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}\right)^{\wedge}\mathbf{J}_{L}\left(\arccos\left(\frac{\left( \left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}}\right)^T\left(\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}\right)}{\norm{\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}}}\norm{\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}}}\right)\frac{\left(\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}}\right) \times \left(\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}\right)}{\norm{\left(\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \mathring{\Vector{}{p}{f}}\right) \times \left(\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}\right)}}\right) & -\hat{E}^{-1}\left(\mathring{\mathbf{P}}\mathring{\mathbf{S}}\right)^{-1} * \Vector{}{p}{f}
        % \end{bmatrix}\tilde{y}
    \end{split}
\end{equation}

\subsubsection*{Case of Fixed Extrinsics}
In the case of fixed extrinsics (non calibrated online) we write
\begin{equation}
    h\left(\phi_{X}\left(\xi\right)\right) = \mathbf{K}L \pi_{Z_1}\left(\mathbf{S}^{-1}C^{-1}\mathbf{P}^{-1} * \Vector{}{p}{f}\right).
\end{equation}
Therefore, the ${\mathbf{C}_t}$ is defined as follows
\begin{equation}
    \begin{split}
        \mathbf{C}_t\varepsilon &= \Fr{\xi}{\hat{\xi}}h\left(\xi\right)\Fr{e}{\mathring{\xi}}\phi_{\hat{X}}\Fr{\varepsilon}{\mathbf{0}}\vartheta^{-1}\left(\varepsilon\right)\left[\varepsilon\right]\\
        &= \mathring{\mathbf{K}}
        \hat{L}
        d_{\pi_{Z_1}}\Gamma\left(\left(\hat{C}\mathbf{S}\right)^{-1}\right)
        \begin{bmatrix}
        \left(\mathring{\mathbf{P}}^{-1} * \hatVector{}{p}{f}\right)^{\wedge} & -\eye_3
        \end{bmatrix}
        \varepsilon_C +
        \mathring{\mathbf{K}}\Xi\left(\hat{L}\pi_{Z_1}\left(\left(\mathring{\mathbf{P}}\hat{C}\mathring{\mathbf{S}}\right)^{-1} * \hatVector{}{p}{f}\right)\right)
        \varepsilon_K.
    \end{split}
\end{equation}

\subsubsection*{Case of Estimated Feature in a Anchor Frame}

==> misc/msceqf/preliminaries.tex <==
\section*{Preliminaries}

\subsection*{Vector and matrix notation}
Vectors describing physical quantities expressed in frame of reference \frameofref{A} are denoted by $\Vector{A}{v}{}$.
Rotation matrices encoding the orientation of a frame of reference \frameofref{B} with respect to a reference \frameofref{A} are denoted by $\Rot{A}{B}$; in particular, $\Rot{A}{B}$ expresses a vector $\Vector{B}{v}{}$ defined in the \frameofref{B} frame of reference into a vector ${\Vector{A}{v}{} = \Rot{A}{B}\Vector{B}{v}{}}$ expressed in the \frameofref{A} frame of reference.
${\eye_n \in \R^{n \times n}}$ denotes the $n$-dim identity matrix, and ${\mathbf{0}_{n \times m} \in \R^{n \times m}}$ denotes the zero matrix with ${n}$ rows and ${m}$ columns.

\subsection*{Useful maps}
For all $\Vector{}{v}{} = \left(x,y,z\right) \in \R^3$, define the maps
\begin{align*}
    &\ubarVector{}{\left(\cdot\right)}{} \AtoB{\R^n}{\R^{n+3}}, 
    &&\Vector{}{v}{} \mapsto \ubarVector{}{v}{} = \left(\mathbf{0}_{3 \times 1}, \Vector{}{v}{}\right) ,\\
    &\lbarVector{}{\left(\cdot\right)}{} \AtoB{\R^n}{\R^{n+3}}, 
    &&\Vector{}{v}{}
    \mapsto \lbarVector{}{v}{} = \left(\Vector{}{v}{}, \mathbf{0}_{3 \times 1}\right) , \\
     &\pi_{Z_1}\left(\cdot\right) \AtoB{\R^{3}}{\R^{3}},
     && \pi_{Z_1}\left(\Vector{}{v}{}\right) \coloneqq \frac{\Vector{}{v}{}}{z},\\
     &\Xi\left(\cdot\right) \AtoB{\R^3}{\R^{3 \times 4}},
     &&\Xi\left(\Vector{}{v}{}\right) = \begin{bmatrix}
     x & 0 & z & 0\\
     0 & y & 0 & z\\
     0 & 0 & 0 & 0
     \end{bmatrix} \in \R^{3 \times 4}.
 \end{align*}
For all $\Vector{}{a}{}, \Vector{}{b}{}, \Vector{}{c}{} \in \R^3 \st (\Vector{}{a}{}, \Vector{}{b}{}, \Vector{}{c}{}) \in \R^9$, define the maps
 \begin{align*}
    &\Pi\left(\cdot\right) \AtoB{\se_2(3)}{\se(3)}, \quad \Pi\left(\left(\Vector{}{a}{}, \Vector{}{b}{}, \Vector{}{c}{}\right)^{\wedge}\right) = \left(\Vector{}{a}{}, \Vector{}{b}{}\right)^{\wedge} \in \se(3), \\
    &\Upsilon\left(\cdot\right) \AtoB{\se_2(3)}{\se(3)}, \quad \Upsilon\left(\left(\Vector{}{a}{}, \Vector{}{b}{}, \Vector{}{c}{}\right)^{\wedge}\right) = \left(\Vector{}{a}{}, \Vector{}{c}{}\right)^{\wedge} \in \se(3),
\end{align*}
For all $X = \left(A, a\right) \in \SE(3) \st A \in \SO(3), a \in \R^3$, define
\begin{equation*}
    \Gamma\left(\cdot\right) \AtoB{\SE(3)}{\SO(3)}, \quad \Gamma\left(X\right) = A \in \SO(3).
\end{equation*}
For all $X = \left(A, a, b\right) \in \SE_2(3) \st A \in \SO(3), a, b \in \R^3$, define
\begin{align*}
    &\chi\left(\cdot\right) \AtoB{\SE_2(3)}{\SE(3)}, \quad \chi\left(X\right) = \left(A, a\right) \in \SE(3),\\
    &\Theta\left(\cdot\right) \AtoB{\SE_2(3)}{\SE(3)}, \quad \Theta\left(X\right) = \left(A, b\right) \in \SE(3).
\end{align*}

\subsection*{Lie Group}
A Lie group $\grpG$ is a smooth manifold endowed with a smooth group multiplication that satisfies the group axioms. For any $X, Y \in \grpG$, the group multiplication is denoted $XY$, the group inverse $X^{-1}$ and the identity element $I$. 

For a given Lie group $\grpG$, $\calG$ denotes the $\grpG$-Torsor\cit{Mahony2013ObserversSymmetry}, which is defined as the set of elements of $\grpG$ (the underlying manifold), but without the group structure.

\subsection*{Lie Algebra}
For a given Lie group $\grpG$, the Lie algebra $\gothg$ is a vector space corresponding to the tangent space at the identity of the group, together with a bilinear non-associative map ${[\cdot, \cdot] \AtoB{\gothg}{\gothg}}$ called Lie bracket. For a matrix Lie group, the Lie-bracket is the matrix commutator, defined by 
\begin{equation*}
    \left[\eta, \kappa \right] = \eta \kappa - \kappa \eta ,
\end{equation*}
for any $\eta, \kappa \in \gothg \subset \R^{n \times n}$.
The Lie algebra $\gothg$ is isomorphic to a vector space $\R^{n}$ of dimension ${n =\mathrm{dim}\left(\gothg\right)}$.
Define the \emph{wedge} map and its inverse, the \emph{vee} map as linear mappings between the vector space and the Lie algebra
\begin{align*}
    &\left(\cdot\right)^{\wedge} \AtoB{\R^{n}}{\gothg} ,\\
    &\left(\cdot\right)^{\vee} \AtoB{\gothg}{\R^{n}} . 
\end{align*} 
For any $X, Y \in \grpG$, define the left and right translation
\begin{align*}
    &\textrm{L}_{X} \AtoB{\grpG}{\grpG}, \qquad \textrm{L}_{X}\left(Y\right) = XY ,\\
    &\textrm{R}_{X} \AtoB{\grpG}{\grpG}, \qquad \textrm{R}_{X}\left(Y\right) = YX . 
\end{align*}

\subsection*{Adjoint Representations}
The Adjoint map for $\grpG$, $\Ad_X \AtoB{\gothg}{\gothg}$ is defined by
\begin{equation*}
    \Adsym{X}{\bm{u}^{\wedge}} = \td \textrm{L}_{X} \td \textrm{R}_{X^{-1}}\left[\bm{u}^{\wedge}\right] ,
\end{equation*}
for every $X \in \grpG$ and ${\bm{u}^{\wedge} \in \gothg}$. $\td \textrm{L}_{X}$, and $\td \textrm{R}_{X}$ are respectively the differentials of the left, and right translation previously defined. 
In the context of matrix Lie group, we can define the Adjoint matrix to be the map ${\AdMsym{X} \AtoB{\R^{n}}{\R^{n}}}$ defined by
\begin{equation*}
    \AdMsym{X}\bm{u} = \left(\Adsym{X}{\bm{u}^{\wedge}}\right)^{\vee} .
\end{equation*}
In addition to the Adjoint map for the group $\grpG$, the adjoint map for the Lie algebra $\gothg$ can be defined as the differential at the identity of the Adjoint map for the group $\grpG$.
The adjoint map for the Lie algebra $\ad_{\bm{u}^\wedge} \AtoB{\gothg}{\gothg}$ is defined by 
\begin{equation*}
    \adsym{\bm{u}^\wedge}{\bm{v}^{\wedge}} = \bm{u}^{\wedge}\bm{v}^{\wedge} - \bm{v}^{\wedge}\bm{u}^{\wedge} = \left[\bm{u}^{\wedge}, \bm{v}^{\wedge}\right] ,
\end{equation*}
that is equivalent to the Lie bracket previously defined. 
In the context of matrix Lie group we can define the adjoint matrix $\adMsym{\bm{u}} \AtoB{\R^{n}}{\R^{n}}$ as 
\begin{equation*}
    \adMsym{\bm{u}}\bm{v} = \left(\bm{u}^{\wedge}\bm{v}^{\wedge} - \bm{v}^{\wedge}\bm{u}^{\wedge}\right)^{\vee} = \left[\bm{u}^{\wedge}, \bm{v}^{\wedge}\right]^{\vee} .
\end{equation*}
The two adjoint operators commute: 
\begin{equation*}
    \Adsym{X}{\adsym{\Vector{}{u}{}^{\wedge}}{\Vector{}{v}{}^{\wedge}}} = \adsym{\left(\Adsym{X}{\Vector{}{u}{}^{\wedge}}\right)}{\Adsym{X}{\Vector{}{v}{}^{\wedge}}} .
\end{equation*}

\subsection*{Group Action and Homogeneous Space}
A right group action of a Lie group $\grpG$ on a differentiable manifold $\calM$ is a smooth map ${\phi \AtoB{\grpG\times \calM}{\calM}}$ that satisfies 
\begin{align*}
    &\phi\left(I, \xi\right) = \xi ,\\
    &\phi\left(X, \phi\left(Y, \xi\right)\right) = \phi\left(YX, \xi\right) ,
\end{align*} 
for any $X,Y \in \grpG$ and $\xi \in \calM$.
A right group action $\phi$ induces a family of diffeomorphism ${\phi_X \AtoB{\calM}{\calM}}$ and smooth nonlinear projections ${\phi_{\xi} \AtoB{\grpG}{\calM}}$. The group action $\phi$ is said to be transitive if the induced projection $\phi_{\xi}$ is surjective, and then, in this case, $\calM$ is termed a homogeneous space.

\subsection*{The Semi-direct Product Group}
A semi-direct product group $\mathbf{G} \ltimes \mathbf{H}$ can be seen as a generalization of the direct product group $\grpG \times \grpH$ where the underlying set is given by the cartesian product of two groups $\grpG$ and $\grpH$, but, contrary to the direct product, in the semi-direct product, the group multiplication is defined with the group $\grpG$ that acts on a group $\grpH$ by a group automorphism. 
Note that the semi-direct product group $\mathbf{G} \ltimes \mathbf{H}$ with the trivial automorphism corresponds to the direct product group $\grpG \times \grpH$.

In this work we will consider a semi-direct product symmetry group $\sdpgrpG := \mathbf{G} \ltimes \gothg$ where $\gothg$ is the Lie algebra of $\grpG$, a vector space group under addition. 
Let $A,B \in \grpG$ and $a,b \in \gothg$ and define $X = \left(A, a\right)$ and $Y = \left(B, b\right)$ elements of the symmetry group $\sdpgrpG$. 
Group multiplication is defined to be the semi-direct product ${YX = \left(BA, b + \Adsym{B}{a}\right)}$. 
The inverse element is ${X^{-1} = \left(A^{-1}, -\Adsym{A^{-1}}{a}\right)}$ and  identity element is ${\left(I, 0\right)}$. 

==> misc/msceqf/triangulation.tex <==
\section*{Feature triangulation}

\subsection*{Linear}
Let ${\Vector{C_j}{p}{f} = \left({^j\mathbf{P}}{^j\mathbf{S}}\right)^{-1} * \Vector{G}{p}{f}}$ denote the feature observed from the camera, and expressed in \frameofref{C_j} frame. $\left({^j\mathbf{P}}{^j\mathbf{S}}\right)$ represent the transformation from frame \frameofref{G} to frame \frameofref{C_j}. 
%
Let ${\Vector{A}{p}{f} = \left({^A\mathbf{P}}{^A\mathbf{S}}\right)^{-1} * \Vector{G}{p}{f}}$ be the feature expressed in a generic anchor frame \frameofref{A} (that can also be the global frame \frameofref{G}), and $\left({^A\mathbf{P}}{^A\mathbf{S}}\right)$ represent the transformation from frame \frameofref{G} to frame \frameofref{A} (that is the identity in the case \frameofref{A} $=$ \frameofref{G}). Then
\begin{align*}
    \Vector{C_j}{p}{f} 
    &= \left({^j\mathbf{P}}{^j\mathbf{S}}\right)^{-1}{^A\mathbf{P}}{^A\mathbf{S}} * \Vector{A}{p}{f}\\
    &= \left({^jE^{-1}}{^AE}\right) * \Vector{A}{p}{f} ,
\end{align*}
where ${^jE}, {^AE}$ are the cloned poses in the symmetry group.

The feature ${\Vector{C_j}{p}{f}}$ can be expressed as ${\Vector{C_j}{p}{f} = ^{C_j}z_f\Vector{C_j}{b}{f}}$, where ${\Vector{C_j}{b}{f}}$ is  the homogeneous vector of normalized ${u, v}$ coordinates, thus
\begin{equation*}
    \Vector{C_j}{p}{f} = \left(^{C_j}z_f\right)\left(\Vector{C_j}{b}{f}\right) 
    = \left(^{C_j}z_f\right)
    \begin{bmatrix}
        ^{C_j}u\\
        ^{C_j}v\\
        1\\
    \end{bmatrix} .
\end{equation*}
\begin{align*}
    \Vector{A}{p}{f} 
    &= \left({^AE^{-1}}{^jE}\right) * \Vector{C_j}{p}{f} \\
    &= \left({^AE^{-1}}{^jE}\right) * \left(^{C_j}z_f\Vector{C_j}{b}{f}\right)\\
    &= \Gamma\left({^AE^{-1}}{^jE}\right)\left(^{C_j}z_f\Vector{C_j}{b}{f}\right) + \left({^AE^{-1}}{^jE}\right) * \Vector{}{0}{}\\
    &= ^{C_j}z_f\Gamma\left({^AE^{-1}}{^jE}\right)\Vector{C_j}{b}{f} + \left({^AE^{-1}}{^jE}\right) * \Vector{}{0}{}\\
    &= ^{C_j}z_f\Vector{A}{b}{f}^j + \left({^AE^{-1}}{^jE}\right) * \Vector{}{0}{} ,
\end{align*}
then, pre-multiplying both sides by ${\left(\Vector{A}{b}{f}^j\right)^{\wedge}}$ yields
\begin{equation*}
    \left(\Vector{A}{b}{f}^j\right)^{\wedge}\Vector{A}{p}{f} = \left(\Vector{A}{b}{f}^j\right)^{\wedge}\left(\left({^AE^{-1}}{^jE}\right) * \Vector{}{0}{}\right) .
\end{equation*}
Therefore, a linear system in the form ${\mathbf{A}\Vector{A}{p}{f} = \mathbf{b}}$ can be built for each of the measurement of the same feature, as follows
\begin{equation*}
    \begin{bmatrix}
        \left(\Vector{A}{b}{f}^1\right)^{\wedge}\\
        \vdots\\
        \left(\Vector{A}{b}{f}^n\right)^{\wedge}
    \end{bmatrix}
    \Vector{A}{p}{f} = 
    \begin{bmatrix}
        \left(\Vector{A}{b}{f}^1\right)^{\wedge}\left(\left({^AE^{-1}}{^1E}\right) * \Vector{}{0}{}\right)\\
        \vdots\\
        \left(\Vector{A}{b}{f}^n\right)^{\wedge}\left(\left({^AE^{-1}}{^nE}\right) * \Vector{}{0}{}\right)
    \end{bmatrix} .
\end{equation*}

Alternatively, we could use two views triangulation (DLT), however, using $n$ views triangulation yields better results.

\subsection*{Nonlinear}
We can formulate a nonlinear least square problem to refine the linear least square solution as follows
\begin{align*}
    \Vector{C_j}{p}{f} 
    &= \left({^jE^{-1}}{^AE}\right) * \Vector{A}{p}{f}\\
    &= \left({^jE^{-1}}{^AE}\right) * \varsigma^{-1}\left(\Vector{}{z}{}\right) ,
\end{align*}
where the anchor frame, and ${\varsigma^{-1}\left(\Vector{}{z}{}\right)}$ depends by the chosen paramterization. Then we can build a nonlinear least square problem with cost given by
\begin{equation*}
    \sum_{j = 1}^{n} \norm{\pi_{S^2}\left(\Vector{j}{uv}{}\right) - \pi_{S^2}\left(\left({^jE^{-1}}{^AE}\right) * \varsigma^{-1}\left(\Vector{}{z}{}\right)\right)}^2 ,
\end{equation*}
where ${\Vector{j}{uv}{}}$ is the direct measurement of the feature in camera $j$ expressed in normalized-uv coordinates.

\emph{Question: What feature parametrization improve the convergence of the nonlinear least square? It is known that the inverse depth parametrization improves it compared to Euclidean parametrization but what about the polar parametrization?}

\textbf{Among all the parametrization discussed, the inverse depth parametrization results in a more stable and faster optimization.}

\subsection*{Ray intersection + Wabba}
When using the polar parametrization we can split the feature triangulation problem into two linear problems.

\subsubsection*{Linear}
the feature ${\Vector{G}{p}{f}}$ is written
\begin{align*}
    \Vector{G}{p}{f} = {^AE} * \Vector{A}{p}{f}
    &= {^jE} * \Vector{C_j}{p}{f} \\
    &= {^jE} * \left(\lambda_j\pi_{S^2}\left(
    \begin{bmatrix}
        ^{C_j}u\\
        ^{C_j}v\\
        1\\
    \end{bmatrix}\right)\right)\\
    &= {^jE} * \lambda_j\pi_{S^2}\left(\Vector{C_j}{b}{f}\right)\\
    {^AE} * \lambda_A\pi_{S^2}\left(\Vector{A}{b}{f}\right)
    &= {^jE} * \lambda_j\pi_{S^2}\left(\Vector{C_j}{b}{f}\right)\\
    \lambda_A\Gamma\left({^AE}\right)\pi_{S^2}\left(\Vector{A}{b}{f}\right) + {^AE}*\Vector{}{0}{}    
    &= \lambda_j\Gamma\left({^jE}\right)\pi_{S^2}\left(\Vector{C_j}{b}{f}\right) + {^jE}*\Vector{}{0}{} .\\
\end{align*}
Then, the following linear problem can be built
\begin{equation*}
    \begin{bmatrix}
        \Gamma\left({^AE}\right)\pi_{S^2}\left(\Vector{A}{b}{f}\right) & -\Gamma\left({^1E}\right)\pi_{S^2}\left(\Vector{C_1}{b}{f}\right) & \cdots & \Vector{}{0}{}\\
        \vdots & \vdots & & \vdots\\
        \Gamma\left({^AE}\right)\pi_{S^2}\left(\Vector{A}{b}{f}\right) & \Vector{}{0}{} & \cdots & -\Gamma\left({^nE}\right)\pi_{S^2}\left(\Vector{C_n}{b}{f}\right)
    \end{bmatrix}
    \begin{bmatrix}
        \lambda_A\\
        \lambda_1\\
        \vdots\\
        \lambda_n
    \end{bmatrix} =
    \begin{bmatrix}
        {^AE}*\Vector{}{0}{} - {^1E}*\Vector{}{0}{}\\
        {^AE}*\Vector{}{0}{} - {^2E}*\Vector{}{0}{}\\
        \vdots\\
        {^AE}*\Vector{}{0}{} - {^nE}*\Vector{}{0}{}
    \end{bmatrix}
\end{equation*}

\subsubsection*{Wabba's problem}
Once a solution for ${\lambda_A,\lambda_1,\cdots,\lambda_n}$ are found, these can be used to build a Wabba's problem.
\begin{align*}
    \Vector{A}{p}{f} 
    &= \left({^AE^{-1}}{^jE}\right) * \Vector{C_j}{p}{f} \\
    \lambda_A{\Rot{}{}}_{Q}^T\mathring{\Vector{}{c}{f}}
    &= \left({^AE^{-1}}{^jE}\right) * \Vector{C_j}{p}{f}\\
    {\Rot{}{}}_{Q}^T\pi_{S^2}\left(\mathring{\Vector{}{c}{f}}\right)
    &= \pi_{S^2}\left(\left({^AE^{-1}}{^jE}\right) * \Vector{C_j}{p}{f}\right) .
\end{align*}
Finally, ${z = \left(\log\left(\frac{1}{\lambda_A}\right), \log\left({\Rot{}{}}_{Q}\right)^{\vee}\right)}$

==> misc/msceqf/vio.tex <==
\section*{Visual Inertial Odometry}

\subsection*{System definition}
Let's assume the existence of a single feature $f$, Then the system's dynamics $\dot{\xi} = f\left(\xi, u\right)$ are
\begin{subequations}
    \begin{align}
        &\dotRot{}{} = \Rot{}{}\left(\ang - \bw\right)^{\wedge} ,\\
        &\dotVector{}{v}{} =  \Rot{}{}\left(\acc - \ba\right) + g\ethree ,\\
        &\dotVector{}{p}{} = \Vector{}{v}{} ,\\
        &\dotVector{}{b}{\omega} = \tauw ,\\
        &\dotVector{}{b}{a} = \taua ,\\
        &\dot{\mathbf{S}} = \mathbf{S}\bm{\mu}^{\wedge} ,\\
        &\dot{\mathbf{K}} = \mathbf{K}\bm{\zeta}^{\wedge} ,\\
        &\dotVector{}{p}{f} = \bm{\nu} .
    \end{align}
\end{subequations}
$\Rot{}{}$ corresponds to the rigid body orientation, $\Vector{}{p}{}$ and $\Vector{}{v}{}$ denote respectively the rigid body position and velocity expressed in the \frameofref{G} frame. $g$ denotes the magnitude of the gravity vector, while $\Vector{}{e}{3}$ denotes the gravity direction in the \frameofref{G} frame. $\ang$ and $\acc$ are the body-fixed, biased, angular velocity and linear acceleration measurements provided by an IMU. $\Vector{}{b}{\omega}$ and $\ba$ are the gyroscope and accelerometer biases respectively. $\bm{\tau}_{\omega}$, $\bm{\tau}_{a}$ are used to model the biases' dynamics, and are zero when the biases are modeled as constant quantities. $\mathbf{S}$ denotes the camera extrinsic calibration, while $\mathbf{K}$ denotes the camera intrinsic calibration. $\Vector{}{p}{f}$ denotes the position of the feature $f$ in the \frameofref{G} frame.

Define ${\mathbf{T} = \left(\Rot{}{}, \Vector{}{v}{}, \Vector{}{p}{}\right)}$ to be the extended pose of the system, and ${\Vector{}{w}{} = \left(\ang, \acc\right)}$ to be the IMU input. Then the system dynamics can be rewritten in compact form as follows
\begin{subequations}
    \begin{align}
        &\dotPose{}{} = \Pose{}{}\left(\mathbf{W} - \mathbf{B} + \mathbf{D}\right) + \left(\mathbf{G} - \mathbf{D}\right)\Pose{}{} ,\\
        &\dotVector{}{b}{} =  \bm{\tau} ,\\
        &\dot{\mathbf{S}} = \mathbf{S}\bm{\mu}^{\wedge} ,\\
        &\dot{\mathbf{K}} = \mathbf{K}\bm{\zeta}^{\wedge} ,\\
        &\dotVector{}{p}{f} = \bm{\nu} .
    \end{align}
\end{subequations}
where the matrices $\mathbf{W}, \mathbf{B}, \mathbf{D}, \mathbf{G}$ are defined as follows
\begin{align*}
    &\mathbf{W} = \lbarVector{}{w}{}^{\wedge} = \begin{bmatrix}
    \ang^{\wedge} & \acc & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \end{bmatrix}\\
    &\mathbf{B} = \lbarVector{}{b}{}^{\wedge} = \begin{bmatrix}
    \bw^{\wedge} & \ba & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \end{bmatrix}\\
    &\mathbf{D} = \begin{bmatrix}
    \mathbf{0}_{3\times 3} & \mathbf{0}_{3\times 1} & \mathbf{0}_{3\times 1}\\
    \mathbf{0}_{1\times 3} & 0 & 1\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \end{bmatrix}\\ 
    &\mathbf{G} = g\ulbarVector{}{e}{3}^{\wedge} = \begin{bmatrix}
    \mathbf{0}_{3\times 3} & g\ethree & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \mathbf{0}_{1\times 3} & 0 & 0\\
    \end{bmatrix}
\end{align*}

The camera measurement is modeled as a bearing measurement of the feature $\Vector{}{p}{f}$. Let ${\mathbf{V} = \left(\Rot{}{}, \Vector{}{v}{}\right)}$ denotes the velocity aided attitude of the system, and ${\mathbf{P} = \left(\Rot{}{}, \Vector{}{p}{}\right)}$ denotes the pose of the system, then the measurement equation is
\begin{align}\label{eq:visualmeas}
    h\left(\xi\right) &= \mathbf{K}\pi_{Z_1}\left(\left(\mathbf{P}\mathbf{S}\right)^{-1} * \Vector{}{p}{f}\right) ,\\
    h\left(\xi\right) &= \pi_{S^2}\left(\mathbf{K}\left(\left(\mathbf{P}\mathbf{S}\right)^{-1} * \Vector{}{p}{f}\right)\right).
\end{align}


Note that the matrix form of the pose ${\mathbf{P}}$ can be computed from the matrix form of the extended pose ${\Pose{}{}}$ as follows
\begin{equation}
    \mathbf{P} = \mathbf{\Gamma}\Pose{}{}\mathbf{\Gamma}^T = 
    \begin{bmatrix}
    \eye_{3} & 0 & 0\\
    \Vector{}{0}{1 \times 3} & 0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \Rot{}{} & \Vector{}{v}{} & \Vector{}{p}{}\\
    \Vector{}{0}{1 \times 3} & 1 & 0\\
    \Vector{}{0}{1 \times 3} & 0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \eye_{3} & \Vector{}{0}{3 \times 1}\\
    0 & 0\\
    0 & 1
    \end{bmatrix}
\end{equation}

==> preamble/preamble_compatible.tex <==

% Colour.  Used mostly for todos/notes/audits.
\usepackage{xcolor}  % Needed for colours - load before mdframed

%% RM Commenting process
%===================================================
%% comment environments {audit}
% audit.  Its an environment used for large chunks of text
\newenvironment{audit}{\color{orange}}{\color{black}}
% todo - use for a reminder of things to do.
\newcommand{\todo}[1]{{\color{red} #1}}
%% aside - a short comment to the authors, but not requiring work.
\newcommand{\aside}[1]{{\color{blue} #1}}
%% \margin{...} % a very short comment put in the margin.
\newcommand{\margin}[1]{\marginpar{\tiny #1}}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Uncomment to switch off notes
%\renewcommand{\margin}[1]{} %% Get rid of all margin comments
%\renewcommand{\todo}[1]{}%%  Get rid of todo comments
%\renewenvironment{audit}{}{} %% leave the audit text but without the colour.
%\renewcommand{\aside}[1]{} %% Get rid of all comments
%===================================================

% math symbols 
\usepackage{amssymb}
% We did use MnSymbol but this had problems with type 3 fonts.

\usepackage{amsmath}
\usepackage{mathdots}

%  this is used for \mathclap and symbol generation needed for \obb symbol.
\usepackage{mathtools} 

% for \mathbb
%\usepackage{bbm}
%\let\mathbb\mathbbm

% left indices
\usepackage{tensor}

% for \mathcal lower case
\usepackage{urwchancal}
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.10] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% allow the use of scalable vector graphics
\usepackage{graphicx}
\usepackage{ifpdf}
\ifpdf
\usepackage{epstopdf}
\epstopdfsetup{update,prepend}
\PrependGraphicsExtensions{.svg}
\DeclareGraphicsRule{.svg}{pdf}{.pdf}{% <- do not remove!
  `inkscape -z -D #1 --export-pdf=\noexpand\OutputFile
}
\fi
%% To switch off figures -
%\usepackage[demo]{graphicx} % use this to switch off figures


% theorem environments
%\usepackage{amsthm}
% -- or
%\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

% list environments
\newenvironment{List}
{\begin{list}
 {[\arabic{enumi}]}
 {\usecounter{enumi}
  \settowidth{\labelwidth}{[99]}}
  \setlength{\labelsep}{1em}}
{\end{list}}

